Correlators on the Wilson Line Defect CFT

Conformal field theory (CFT) plays a key role in modern theoretical physics. Through CFT we describe real physical systems at criticality and fixed points of the renormalization group flow. It is also central in the study of quantum gravity, thanks to the AdS/CFT correspondence. This thesis originates in the context of the N=4 supersymmetric Yang-Mills (SYM) theory, which represents the CFT side of this correspondence. This work mainly revolves around the supersymmetric Wilson line and its interpretation as a conformal defect in N=4 SYM. Particularly, we focus on excitations localized on the defect called insertions, whose correlators are described by a one-dimensional CFT. The first main result of this work is an efficient algorithm for computing multipoint correlation functions of scalar insertions on the Wilson line, consisting of recursion relations up to next-to-leading order at weak coupling. We show various computations of such four-, five- and six-point correlators, and discuss their properties. Moreover, we use the four-point function case to illustrate the power of the Ward identities, which are crucial in deriving a next-to-next-to-leading order result. Thanks to these perturbative results, we find a family of differential operators annihilating our correlation functions, which we conjecture to be a multipoint extension of the Ward identities satisfied by the four-point functions. These non-perturbative constraints are shown to be fundamental ingredients in the bootstrap of a five-point function at strong coupling. To conclude, we define an inherently one-dimensional Mellin amplitude at the non-perturbative level with appropriate subtractions and analytical continuations. The efficiency of the 1d Mellin formalism is manifest at the perturbative level. We find a closed-form expression for the Mellin transform of leading order contact interactions and use it to extract CFT data.

==> Figures/commands.tex <==
%% DEFINE MATH COMMANDS
%Sign function
\DeclareMathOperator{\sgn}{sign}
%Pfaffian
\newcommand{\Pf}{\text{Pf}\ }
%Trace
\newcommand{\Tr}{\text{tr}\ }
%Super-Pfaffian
\newcommand{\SPf}{\text{SPf}\ }
%Dilogarithm
\newcommand{\Li}{{\normalfont\text{Li}}}
%Operators
\newcommand{\Op}{\mathcal{O}}
\newcommand{\NOp}{\mathcal{N}}
\newcommand{\Oh}{\hat{\mathcal{O}}}
\newcommand{\Nh}{\hat{\mathcal{N}}}
\newcommand{\Kh}{\hat{\mathcal{K}}}
\newcommand{\Ph}{\hat{\mathcal{P}}}
\newcommand{\bh}{\hat{b}}
\newcommand{\uh}{\hat{u}}
\newcommand{\phat}{\hat{p}}
\newcommand{\Jh}{\hat{J}}
\newcommand{\alphah}{\hat{\alpha}}
\newcommand{\idh}{\hat{\mathds{1}}}
\newcommand{\id}{\mathds{1}}
\newcommand{\Wl}{\mathcal{W}_\ell}
\newcommand{\Wc}{\mathcal{W}_c}

\newcommand{\eqn}[1]{eq.~(\ref{#1})}
\newcommand{\vvev}[1]{\langle\!\langle\, #1 \, \rangle\!\rangle}
\newcommand{\vev}[1]{\langle\, #1 \, \rangle}

%% HELP FUNCTION FOR DIAGRAMS: gluon lines are symmetric
\newif\ifstartcompletesineup
\newif\ifendcompletesineup
\pgfkeys{
    /pgf/decoration/.cd,
    start up/.is if=startcompletesineup,
    start up=true,
    start up/.default=true,
    start down/.style={/pgf/decoration/start up=false},
    end up/.is if=endcompletesineup,
    end up=true,
    end up/.default=true,
    end down/.style={/pgf/decoration/end up=false}
}
\pgfdeclaredecoration{complete sines}{initial}
{
    \state{initial}[
        width=+0pt,
        next state=upsine,
        persistent precomputation={
            \ifstartcompletesineup
                \pgfkeys{/pgf/decoration automaton/next state=upsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5*\pgfdecoratedinputsegmentlength / (ceil(0.5* \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) )
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.499)
                    }
                \fi
            \else
                \pgfkeys{/pgf/decoration automaton/next state=downsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5* \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.4999)
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) )
                    }
                \fi
            \fi
            \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
        }] {}
    \state{downsine}[width=\pgfdecorationsegmentlength,next state=upsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
    }
    \state{upsine}[width=\pgfdecorationsegmentlength,next state=downsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
}
    \state{final}{}
}


%% DEFINE STYLE OF PROPAGATORS
%define color for background box
\definecolor{bgbox}{RGB}{255,254,230}
%define color for setup plane
\definecolor{setupplane}{RGB}{230,230,230}
%define color for gluon line
\definecolor{gluoncolor}{RGB}{207,54,108}
%define color for vertex
\definecolor{vertexcolor}{RGB}{53,152,219}
%define color for self-energy
\definecolor{SEcolor}{RGB}{176,156,255}
%define color for blob
\definecolor{blobcolor}{RGB}{190,180,230}
\tikzset{
%Scalar
corner/.style={line width=1pt,dashed,draw=black,dash pattern=on 6pt off 4pt},
%Fermion
scalar/.style={line width=1pt,draw=black},
%Gluon
gluon/.style={line width=1pt,decorate, draw=gluoncolor,
    decoration={complete sines,aspect=0,amplitude=1.25mm,segment length=1.5mm,start up,end up}},
%Ghost
ghost/.style={line width=1pt,loosely dotted,draw=black},
%Wilson Line
wilson/.style={line width=2pt,draw=black},
 }
%Define semiloops for diagrams
\NewDocumentCommand\semiloop{O{black}mmmO{}O{above}}
{%
\draw[#1] let \p1 = ($(#3)-(#2)$) in (#3) arc (#4:({#4+180}):({0.5*veclen(\x1,\y1)})node[midway, #6] {#5};)
}

%% Calligraphic letters
%\def\Am{{\mathcal{A}}}
%\def\Bm{{\mathcal{B}}}
%\def\Cm{{\mathcal{C}}}
%\def\Dm{{\mathcal{D}}}
%\def\Em{{\mathcal{E}}}
%\def\Fm{{\mathcal{F}}}
%\def\Gm{{\mathcal{G}}}
%\def\Hm{{\mathcal{H}}}
%\def\Im{{\mathcal{I}}}
%\def\Km{{\mathcal{K}}}
\def\Lm{{\mathcal{L}}}
%\def\Mm{{\mathcal{M}}}
%\def\Nm{{\mathcal{N}}}
%\def\Om{{\mathcal{O}}}
%\def\Pm{{\mathcal{P}}}
%\def\Qm{{\mathcal{Q}}}
%\def\Rm{{\mathcal{R}}}
%\def\Sm{{\mathcal{S}}}
%\def\Um{{\mathcal{U}}}
%\def\Xm{{\mathcal{X}}}
%\def\Zm{{\mathcal{Z}}}
%
% Barred generators
\def\Mb{{\bar{M}}}
\def\Qb{{\bar{Q}}}
\def\Sb{{\bar{S}}}
%
% Indices with/without dots
\def\a{{\alpha}}
\def\b{{\beta}}
\def\c{{\gamma}}
\def\d{{\delta}}
%\def\ad{{\dot{\alpha}}}
\def\bd{{\dot{\beta}}}
\def\cd{{\dot{\gamma}}}
%\def\dd{{\dot{\delta}}}
%
% Weird supercharge
\usepackage{bbm}
\newcommand\QQ{\mathbbmtt{Q}}
\newcommand\QQd{\mathbbmtt{Q}^\dagger}

% Other
\def \ph{\phantom}
\def\veps{\varepsilon}
%\DeclareMathOperator{\tr}{tr}
\newcommand\yb{{\bar{y}}}
\newcommand\zb{{\bar{z}}}
\newcommand\g{{\gamma}}
\newcommand\gb{{\bar\gamma}}
%\newcommand\Dh{{\hat{\Delta}}}
%\newcommand\Dp{{\Delta_\phi}}
\newcommand{\Otop}[1]{{\Om^\mathrm{top}_{#1}}}
\newcommand{\Ohtop}[1]{{\widehat{\Om}^\mathrm{top}_{#1}}}
\def\wh{\widehat}


==> Figures/packages.tex <==
\usepackage{slashed} % for Feynman slashed notation
\usepackage{mathtools} % for subequation numbering
\usepackage{tikz}
\usepackage{dsfont} % for displaying the blackboard 1 properly
\usetikzlibrary{positioning,arrows,calc}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{patterns}
\usepackage{xparse}
\usepackage{diagbox} % for category cells in tables
\usepackage{tensor} % for typesetting mixed tensor indices
\usepackage{subcaption} % to use subfigure environment (pics side by side)
\usepackage{float}

==> packages.tex <==

\usepackage[utf8]{inputenc} % Required for inputting international characters
\usepackage[T1]{fontenc} % Output font encoding for international characters
\usepackage{amsmath, amssymb, graphics}
\usepackage{lmodern} %font
\usepackage[english]{babel} % Required for automatically changing names of document elements to languages besides english
%\usepackage{cite}
\RequirePackage{scrbase} % Required for handling language-dependent names of sections/document elements
\RequirePackage{scrhack} % Loads fixes for various packages
\RequirePackage{setspace} % Required for changing line spacing
\RequirePackage{longtable} % Required for tables that span multiple pages (used in the symbols, abbreviations and physical constants pages)
\RequirePackage{siunitx} % Required for \SI commands
\RequirePackage{graphicx} % Required to include images
\graphicspath{{Figures/}{./}} % Specifies where to look for included images
\RequirePackage{booktabs} % Required for better table rules
\usepackage[margin=0cm, labelfont=bf]{caption} % Required for customising the captions
\usepackage{subcaption} % to use subfigure environment (pics side by side)

\usepackage{tensor}

\renewcommand\thefootnote{\textcolor{mypinegreen}{\arabic{footnote}}} %footnote color

\usepackage{etoolbox}
\patchcmd{\part}{\thispagestyle{plain}}{\thispagestyle{empty}}{}{}

%----------------------------------------------------------------------------------------
%	COLOURS
%----------------------------------------------------------------------------------------

\usepackage[dvipsnames]{xcolor} % Required for specifying custom colours
\definecolor{mypinegreen}{HTML}{00675A}

%----------------------------------------------------------------------------------------
%	ADDITIONAL PACKAGES
%----------------------------------------------------------------------------------------

\usepackage[autostyle=true]{csquotes} % Required to generate language-dependent quotes in the bibliography
\usepackage{verbatim} %to allow commenting sections
\usepackage{fancyhdr} %to use fancy as a style of the page
\usepackage{lipsum}
\usepackage[Sonny]{fncychap} %chapter style
\usepackage{amssymb,amsmath} %for formulas
\usepackage[nottoc]{tocbibind} %include references in the table of contents
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=mypinegreen,          % color of internal links (change box color with linkbordercolor)
    citecolor=mypinegreen,
    filecolor=mypinegreen,      % color of file links
    urlcolor=mypinegreen
    }
\usepackage[numbered]{bookmark}
\usepackage{epsfig}
\usepackage{graphics, tikz}
\usepackage[multiple]{footmisc}
\usepackage{fancybox,framed,tikz}
\usetikzlibrary{decorations.pathmorphing,patterns}
\usepackage{dsfont}
\usepackage{mathtools} % for subequation numbering
\usepackage{braket} 
\usepackage{slashed} % for Feynman slashed notation
\usepackage{rotating}
\usepackage{bbold,amsfonts}
\usepackage{multirow}
\usepackage{upgreek}
\usepackage{amsfonts,euscript,amssymb,stmaryrd,braket}
\usetikzlibrary{shapes.misc,arrows,decorations.markings,patterns}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{bbold,bbding}
\usepackage{amsthm} 
\usepackage{esint}
\usepackage{simpler-wick} %for Wick contractions
\usepackage{tensor} % for typesetting mixed tensor indices
\usepackage{dsfont} % for displaying the blackboard 1 properly
\usetikzlibrary{positioning,arrows,calc}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{patterns}
\usepackage{xparse}
\usepackage{diagbox} % for category cells in tables
\usepackage{tensor} % for typesetting mixed tensor indices
\usepackage{url} %to have urls with special characters
\usepackage{bibentry} %to cite fully paper in main text
%\usepackage[square,sort,comma,numbers]{natbib} %to make bibentry work
\usepackage[numbers,sort&compress]{natbib}
\usepackage{mathtools} %to write stuff over/under arrow

\newtheorem{theorem}{Theorem}

\tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={1pt}}


